ObjectNav Revisited: On Evaluation of Embodied Agents Navigating to Objects

We revisit the problem of Object-Goal Navigation (ObjectNav). In its simplest form, ObjectNav is defined as the task of navigating to an object, specified by its label, in an unexplored environment. In particular, the agent is initialized at a random location and pose in an environment and asked to find an instance of an object category, e.g., find a chair, by navigating to it. As the community begins to show increased interest in semantic goal specification for navigation tasks, a number of different often-inconsistent interpretations of this task are emerging. This document summarizes the consensus recommendations of this working group on ObjectNav. In particular, we make recommendations on subtle but important details of evaluation criteria (for measuring success when navigating towards a target object), the agent's embodiment parameters, and the characteristics of the environments within which the task is carried out. Finally, we provide a detailed description of the instantiation of these recommendations in challenges organized at the Embodied AI workshop at CVPR 2020 http://embodied-ai.org .

==> sections/2_related_work.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%We discuss work focusing on themes related to our contributions: 3D simulation platforms, embodied AI tasks making use of simulation, and simulation-to-reality transfer for embodied AI.



==> sections/4_objectnav_task_instantiations.tex <==
\section{ObjectNav Task Specifications}
In this Section we propose a concrete specification of an ObjectNav task.
\subsection{Embodiment}
The experiments by Savva~\etal~\cite{habitat19iccv} 
and the Habitat Challenge 2019 \cite{habitat_challenge} modelled 
the agent as an idealized cylinder 
of radius $0.1$m and height $1.5$m. 
As shown in \figref{fig:simvreal}, 
we configure the agent to match 
the \locobot robot as closely as possible.
Specifically, we configure the simulated agent's base-radius and height to be $0.18\text{m}$ and $0.88\text{m}$ respectively. 


\xhdr{Action Space.} \label{action_space}
The action space for the agent consists of 6 actions: 
\texttt{move-forward 0.25m}, 
\texttt{turn-left 30$^{\circ}$}, 
\texttt{turn-right 30$^{\circ}$},  
\texttt{look-up 30$^{\circ}$},  
\texttt{look-down 30$^{\circ}$}
and \texttt{STOP}.
Note that in contrast to \cite{habitat19iccv, habitat_challenge}, 
we increased the angles associated with \texttt{turn-left} and \texttt{turn-right} actions from $10^{\circ}$ to $30^{\circ}$ degrees due to the concerns described 
in \cite{kadian_cvpr20}. 
Furthermore, in \cite{habitat19iccv, habitat_challenge}, 
agent actions are deterministic -- \ie when the agent executes \texttt{turn-left 30$^{\circ}$}, it turns \emph{exactly} $30^\circ$, and \texttt{forward 0.25\text{m}} moves the agent \emph{exactly} $0.25\text{m}$ forward (modulo collisions).
However, no robot moves deterministically due to real-world actuation noise.  
To model the actions on \locobot, we leverage an actuation noise model derived from mocap-based benchmarking 
by the PyRobot authors~\cite{pyrobot2019}. 
Specifically, when the agent calls (say) \texttt{forward}, 
we sample from 
an action-specific 2D Gaussian distribution over relative displacements. \figref{fig:noisy-actions} shows  
trajectory rollouts sampled from this noise model
(in a Gibson\cite{xia2018gibson} home). 
As shown, identical action sequences can lead to vastly different final locations.

\xhdr{Sensor Specification.}
The agent is equipped with an RGB-D camera and a (noiseless) GPS+Compass sensor. 
We attempt to match the camera specification in simulation to the Azure Kinect camera. Specifically, 
we set the camera's horizontal field of view to $79^{\circ}$, resolution to VGA (height $\times$ width = 480 $\times$ 640 pixels),  
and 
depth sensing clipped to a minimum and maximum of $0.5$m and $6$m respectively. The camera's pose is initialized tilted down 
(negative elevation angle of 30$^{\circ}$) to avoid a blind spot right in front of the agent. 
The GPS+Compass sensor provides relative location ($x, y, z$) and heading (azimuth angle) \wrt 
the agent's start location (origin) and heading ($0^\circ$). Thus, the agent's random spawn location and pose establishes 
a coordinate system for that episode. 


\xhdr{Collision Dynamics and `Sliding'.}
In prior work \cite{habitat19iccv, habitat_challenge}, 
%In Habitat-Sim~\cite{habitat19iccv}, 
when the agent takes an action that results in a collision, the agent \emph{slides} along the obstacle as opposed to stopping.
This behavior is prevalent in video game engines as it allows for smooth human control; it is also enabled by default in MINOS~\cite{savva2017minos}, Deepmind Lab~\cite{beattie2016deepmind}, AI2 THOR~\cite{ai2thor}, and Gibson~\cite{xia2018gibson} v1. In recent work~\cite{kadian_cvpr20}, we have found that this behavior 
enables `cheating' by learned agents.
Specifically, as illustrated by an example in \figref{fig:corner-clipping}, 
the agent exploits this sliding mechanism to take an effective path that appears to travel \emph{through non-navigable regions} of the environment (like walls).  
Such policies fail disastrously in the real world where the robot bump sensors  force a stop on contact with obstacles. 
%This sliding issue is also 
To rectify this issue, we modify Habitat-Sim to %allow for 
disable sliding on collisions. 

\subsection{Environments}
We propose to use photorealistic environments. Currently, there are several existing visual assets which are appropriate for ObjectNav.
\subsubsection{Matterport3D} \label{matterport}
We propose to use 90 of the Matterport3D scenes (MP3D)~\cite{matterport} with the standard splits of train/val/test as prescribed by Anderson \etal \cite{anderson2018evaluation}. Note that as in recent works, 
there is no overlap between train, val, and test scenes.

MP3D40 contains 40 categories annotated, which includes objects (\eg doors), floor-plan elements (\eg counter tops), \etc. 
We hand-select a subset of object categories by excluding various categories that are not visually well defined like doorways or windows and trivial cases like walls, floors, and ceilings.
In total, our subset contains 21 categories with 50851 instances 
in 90 environments, 
with an average of categories/instances per environment for the training split.  

We create ObjectGoal navigation episode-datasets for Matterport3D. 
An episode is defined by the unique id of the scene, 
the starting position and orientation of the agent, and the goal category label. Additional metadata such as the Euclidean distance and the geodesic distance along the shortest path (GDSP) from start position to goal position is also included. All valid goal viewpoints are also included which each episode.
We restricted the maximum action length of the shortest action path to 750 + checked the ratio of geodesic to euclidean distance.

Success zone for the goal object is calculated as positions from which the object can be visible with $\leq 1m$ distance to bounding box of the goal object. To optimize success and distance to goal calculations we provide navigable points in success zone as episode specification for each goal object and call it viewpoints. The viewpoints were sampled with $\frac{R_{agent}}{2}$ grid.

We attempt to be as descriptive as possible about these seemingly low-level but important choices. 
A complete config is available here: 
\url{https://github.com/facebookresearch/habitat-challenge/blob/challenge-2020/habitat-challenge-data/challenge_objectnav2020.local.rgbd.yaml}
which we hope will help iron out any inconsistencies. 

\subsubsection{Gibson}
Another set of 3D scans of real homes is Gibson~\cite{xia2018gibson}. This dataset currently contains $572$ environments, of which only a subset has been semantically labeled with objects classes. In particular, Armeni et al.~\cite{armeni20193d} provides object segmentations and labels on $35$ homes. This dataset comes with a following split: $25$ homes for training, $5$ for validation, and $5$ for testing. Note that many of the homes have multiple floors, which we treat as disjoint spaces. For example, the test set has $12$ floors total. 

We suggest to use 9 objects: `bed', `chair', `microwave', `refrigerator', `table', `toilet', `oven', `tv', 'sofa', which are the most common ones among the ones present in the dataset.

\subsubsection{AI2-THOR} AI2-THOR \cite{ai2thor} consists of a set of near-photo-realistic scenes that are designed by 3D artists. AI2-THOR currently includes two frameworks iTHOR and RoboTHOR. iTHOR is a synthetic platform mainly designed for interacting with objects and changing their state based on the physical properties of the objects and scenes. RoboTHOR consists of a set of scenes in simulation as well as the real world. The main purpose of RoboTHOR is to evaluate the generalization of models from simulation to the real world. In total, iTHOR and RoboTHOR currently have 209 scenes and 115 object categories which can be repositioned programatically to generate new configurations in the scenes. Both iTHOR and RoboTHOR have been used a platform for the ObjectNav task \cite{yang19,wortsman19,robothor}.



